Minimal Solvers for Mini-Loop Closures in 3D Multi-Scan Alignment

3D scan registration is a classical, yet a highly useful problem in the context of 3D sensors such as Kinect and Velodyne. While there are several existing methods, the techniques are usually incremental where adjacent scans are registered first to obtain the initial poses, followed by motion averaging and bundle-adjustment refinement. In this paper, we take a different approach and develop minimal solvers for jointly computing the initial poses of cameras in small loops such as 3-, 4-, and 5-cycles. Note that the classical registration of 2 scans can be done using a minimum of 3 point matches to compute 6 degrees of relative motion. On the other hand, to jointly compute the 3D registrations in n-cycles, we take 2 point matches between the first n-1 consecutive pairs (i.e., Scan 1 & Scan 2, ... , and Scan n-1 & Scan n) and 1 or 2 point matches between Scan 1 and Scan n. Overall, we use 5, 7, and 10 point matches for 3-, 4-, and 5-cycles, and recover 12, 18, and 24 degrees of transformation variables, respectively. Using simulations and real-data we show that the 3D registration using mini n-cycles are computationally efficient, and can provide alternate and better initial poses compared to standard pairwise methods.

==> files/introAllRefs.tex <==
\section{Introduction}

Many geometers working on algebraic minimal solvers would have attempted to solve the notorious and classical 3-view 4-point relative pose estimation. Given 4 triplets of point matches, the goal is to jointly find the poses of the 3 cameras. There has been some great progress on this problem using one-dimensional search~\cite{Nister2006} and semi-definite programming~\cite{Li2010}, but we still don't have the simple and direct minimal algebraic solver that we usually derive for most geometric vision problems. If one manages to solve this problem for RGB cameras, what would be the next big challenge? Should we next look at the 4-view 3-point relative pose problem? While there has been a great deal of effort to solve this higher-order pose estimation problems in the case of RGB cameras, the equivalent problem with RGBD cameras has received no attention. In the case of RGBD sensors, the n-camera relative pose problem is relatively less notorious till $n=5$, and even practically deployable. At this point, when the price point for commercial RGBD sensors is decreasing due to the progress in robotics and self-driving industry, it would be a good time to fully equip the arsenal with algebraic minimal solvers for depth sensors. 

\begin{figure}
    \centering
    \includegraphics[width=0.49\textwidth]{figs/fig0v2.jpg}
    \caption{\emph{Minimal solutions for loop closures in 3D scan registration. At the left we show four point clouds and seven 3D point correspondences between within the point clouds: two from Scans1 \&Scan2; two from Scans2 \&Scan3; two from Scans3\&Scan4; and one two from Scans1\&Scan4. We show the registered pointcloud using our minimal solver for 4-cycle that jointly computes the pose parameters for all the four cameras.}}
    \label{fig:intro}
\end{figure}

Consider Fig.~\ref{fig:intro} where we show four different scans collected using a Kinect sensor. We compute point correspondences between adjacent scans. We jointly compute the poses of all four cameras using a minimal solver that uses a total of 7 point matches (2 from Scans1 \&Scan2; 2 from Scans2 \&Scan3; 2 from Scans3\&Scan4; and 1 two from Scans1\&Scan4). Using these 7 point correspondences, we are able to compute 18 degrees of pose variables, and the points from all the four scans are registered as shown in Fig.~\ref{fig:intro} (at the right). Previous methods for RGBD registration typically employ pair-wise registration where the initial poses are computed between pairs of cameras, and a final refinement is done using bundle adjustment. Note that the pairwise methods (see Orthogonal Procrustes problem \cite{schonemann66} that uses a minimum of 3 point matches) typically accumulate drift even in mini $n$-cycles, where $n > 2$. Our formulation naturally eliminates the drift in these mini $n-$cycles, and thereby provide better pose parameters. This paper systematically studies the possibility of joint pose estimation for mini $n-$cycles derives algebraic minimal solvers, which are typically embedded in a Random Sample Consensus (RANSAC)~\cite{fischler1981} framework for robust estimation of pose parameters. It has been well established that minimal solvers tend to perform robustly in the presence of outliers. 

%\noindent
%{\bf Overview of the paper:}
%We survey the related work for 3D scan alignment and minimal solvers in computer vision. In Sec.~\ref{sec:camera_solvers} we present our solvers and Sec.~\ref{sec:planar} shows the planar motion case.
%The pose graph refinement is shown in Sec.~\ref{sec:pose_refinement}. We show results with synthetic and real data in Sec.~\ref{sec:results}, and discuss the results in Sec.~\ref{sec:discussion}.

\iffalse
{\color{blue}
Some minimal solvers in the literature for absolute/relative pose problems


Hybrid pose estimation by Pollefeys where they combine 2D and 3D matches. 

Check out the papers from usual suspects on 3D SLAM: It would be worth checking the websites of Venu, Hongdong, {\color{red}Pollefeys}, Daniel Cremers, Koltun, Kinect-based papers, {\color{red}Yasu Furukawa}.

Survey some registration with hybrid primitives (planes and lines). 

Survey some methods on 3-view 4-point problem in the context of RGB cameras, and question why an equivalent problem in 3D sensors was never considered? 

% The goal in this paper... consider more than two cameras in the relative 3D pose estimation, to minimize the drift between the cameras
}
\fi

\subsection{Related Work}
We carefully survey some of the classical and modern registration algorithms that employ 3D sensors. 

\vspace{0.4cm}\noindent{\bf 3D Scan Alignment:~}
The classic approach to solve the 3D scan alignment problem is the Iterated Closest Point (ICP) algorithm, proposed in \cite{besl92,zhang92}. Over the years, several efficient and robust solutions have been proposed in the literature to solve the 3D multi-scan alignment using 3D point, such as \cite{trucco99,fitzgibbon03,tsin04,chetverikov05,jian05,rusu09,segal09,myronenko10,newcombe11,yang13,venu14,li17,park17}. Recently, also using 3D points, in~\cite{bustos16} authors propose a fast and efficient technique for 3D rotation search in 3D scans alignment.

Besides the classic approach presented above, recently several authors have been proposing alternatives using more information about the observed 3D scene. In \cite{endres14}, it was introduced a beam-based environment measurement model that allows the evaluation the quality of a frame-to-frame estimation.
For example, in \cite{taguchi13,raposo13,ma16,hsiao17,bhattacharya17,liu18} authors propose the use of 3D planes to improve the SLAM using 3D cameras. In \cite{lu15} authors extract and use 3D straight lines for 3D SLAM, while in \cite{choi13} authors used edge detection. In \cite{halber17}, authors proposed a more general scheme that detects and enforces constraints (geometric relationships and feature correspondences). Surveys on the evaluation of 3D SLAM methods were presented in~\cite{endres12,sturm12}.

% non-rigid 3D registration
Usually, when computing the transformation that aligns 3D scans, one assume that the world is static in the acquisition of the data. This is a common assumption in many of solver for the relative/absolute pose problems. However, similar to the use of RGB images, some authors proposed solvers for the non-rigid 3D registration problem (see for example \cite{li08,zollhofer12,bernard17,slavcheva17,ma17}). A survey on rigid and non-rigid registration of 3D point clouds is presented in \cite{tam13}.

% papers on semantics + 3D registration
In addition to finding the 3D transformations that align 3D scans, there has been some developments on doing both the 3D registration and semantic segmentation using RGB-D images. Recently, several works were proposed such as \cite{tatarchenko18,schonberger18,zaganidis18,zeng18}.

Recently, some deep learning techniques techniques were used in order to get a better 3D registrations.
In \cite{elbaz17} it was proposed to encode local 3D geometric structures using a deep neural network auto-encoder.
\cite{ma17,tatarchenko18} propose the use of a deep neural network approach to predict semantic segmentation from RGB-D sequences. In \cite{khoury17} authors propose a new method for learning compact geometric features. \cite{liu18} proposes the a deep neural architecture to to automatically reconstruct floor-plans. In \cite{zeng18}, authors proposed a model that recovers the geometry with semantically segmented architectural components, which is given by a deep neural networks.

\vspace{0.4cm}\noindent{\bf Minimal Solvers:~}
Minimal solvers is one of the more active topics in 3D computer vision, with several work published in the last years. There are several solvers already proposed in the literature. However, most of them are for 2D images (RGB cameras).

% absolute
Several solutions were proposed for the absolute pose for central perspective cameras (three 3D point correspondences between the world and image), see for example~\cite{haralick94,gao03,kneip11,ke17,wang18,persson18}. There are also solution that use other types of features, such as lines \cite{dhome89,chen90,ramalingam11}, solvers for multi-perspective cameras 
\cite{gim15,gim16,miraldo18} (using both points and lines), and for pose for other settings such as calibrated systems or \cite{kukelova13,micusik13,wu15}.
The pose estimation has also been studied for the pose and scale of multiperspective systems, such as~\cite{sweeney14,ventura14,camposeco16}.

% relative
When considering the relative pose estimation, several approaches have also been proposed for solving the minimal relative pose problem. See for example \cite{mister04,li06b} for calibrated cameras. There are other solutions such as \cite{li13} which studies the relative pose estimation with a known relative rotation angle, \cite{fraundorfer10,saurer15} for the relative pose with known directions, \cite{stewenius05b,li06} for the relative pose with unknown focal length, solutions invariant to translation \cite{kneip12}, and solutions to the generalized relative pose problem \cite{stewenius05c,ventura15}.
In \cite{camposeco18}, authors presented an hybrid minimal solvers that combine relative with absolute poses.

\textcolor{blue}{SR: The literature survey looks great, but I feel that we should cut down the list for the CVPR submission. It might be great for a journal or survey paper later.}

\subsection{Notation and Problem Definition}\label{sec:prob_definition}
For simplicity, we use $\{n\}$ to denote Scan $n$.
The $i$\textsuperscript{th} 3D point in $\{n\}$ is denoted as $\mathbf{p}_i^{\{n\}}\in\mathbb{R}^4$, which is represented in homogeneous coordinates. Rotation matrices and translation vectors are denoted as $\mathbf{R}^{\{n,m\}}\in\mathcal{SO}(3)$ \& $\mathbf{t}^{\{n,m\}}\in\mathbb{R}^3$, respectively (we use $\{n,m\}$ to denote the transformation from $\{n\}$ to $\{m\}$).
We use the N-loop to denote the sequences of N 3D scans with loop closure (first and last point clouds in the sequence have 3D point correspondences).

This paper aims at estimating the rigid transformation between a sequence of RGB-D images (colored 3D point cloud).
The goal is to find the transformation matrices $\mathbf{T}^{\{n,m\}}\in\mathcal{SE}(3)$ that transform 3D points from coordinate system $\{n\}$ to $\{m\}$ such that
\begin{equation}
    \mathbf{p}_i^{\{m\}}
    =
    \underbrace{\begin{bmatrix}
    \mathbf{R}^{\{n,m\}} & \mathbf{t}^{\{m,m\}} \\
    \mathbf{0}_{1,3} & 1 
    \end{bmatrix}}_{\mathbf{T}^{\{n,m\}}}
    \mathbf{p}_i^{\{n\}},
\end{equation}
for all the available $\{n\}$ and $\{m\}$ such that $n\neq m$.

\subsection{Our Contributions}

We summarize our contributions below:

\begin{itemize}
    \item We propose minimal solvers for the mini $n$-cycles in 3D point cloud registration. We propose four new solvers for 3-, 4-, and 5-loop cycles in which we need less than three correspondences between each pair of 3D scans (notice the three 3D point case is the minimal case for two scan 3D registration). The Table~\ref{tab:sumup3D} highlights the different $n$-cycles, required point correspondences, and the number of solutions. 
    \item To recover the poses from a large graph, we show graph-based algorithms that allows us to use the different mini $n$-cycles to obtain pose parameters.
\end{itemize}

\begin{table}
\centering
\scalebox{0.73}{
\begin{tabular}{ |c|l|c|c| }
 \hline
 \bf \thead{Loop Cycle \\ \#Cameras} & \multicolumn{1}{c|}{\bf \#Correspondences}  & \bf Total & \bf \#Solutions \\
 \hline\hline
 Two   & $\#\bm{3}\{1,2\} $  & 3 & 2 \\ \hline
 Three & $\#\bm{2}\{1,2\};\ \#\bm{2}\{2,3\}; \ \#\bm{1}\{1,4\} $  & 5 & 4 \\ \hline
 Four  & $\#\bm{2}\{1,2\};\ \#\bm{2}\{2,3\}; \ \#\bm{2}\{3,4\}; \ \#\bm{1}\{1,4\} $ & 7 & 16 \\ \hline
 Five  & $\begin{aligned}\#\bm{2}&\{1,2\};\  \#\bm{2}\{2,3\}; \\ & \#\bm{2}\{3,4\}; \ \#\bm{2}\{4,5\}; \ \#\bm{2}\{1,5\} \end{aligned}$ & 10 & 32 \\ \hline
 {\color{red}\bf Six}   & $\begin{aligned}\#\bm{2}&\{1,2\};\  \#\bm{2}\{2,3\}; \ \#\bm{2}\{3,4\}; \\ & \#\bm{2}\{4,5\}; \ \#\bm{2}\{5,6\}; \ \#\bm{2}\{1,6\}\end{aligned}$ & 12 & {\color{red}\bf 288}\footnotemark \\ \hline
{\color{red}\bf Seven} & $\begin{aligned}\#\bm{2}&\{1,2\};\  \#\bm{2}\{2,3\}; \#\bm{2}\{3,4\}; \ \#\bm{2}\{4,5\}; \\ &  \#\bm{2}\{5,6\}; \ \#\bm{2}\{6,7\}; \ \#\bm{2}\{1,7\} \end{aligned}$ & 14 & {\color{red}\bf  XX}\footnotemark[\value{footnote}]\\ \hline
\end{tabular}}
\caption{\emph{This table summarizes the minimal number of correspondences requires to compute the pose using three or more than three points to compute the 3D point registration. In the table, $\#\bm{i}\{j,k\}$ means $i$ point correspondences within the sequence of point clouds $\{j,k\}$.}}
\label{tab:sumup3D}
\end{table}
\footnotetext{High number of solutions will lead to unstable ones, as reported in several works such as~\cite{camposeco18,sweeney15}.}
